Data-Driven Program Completion

We introduce program splicing, a programming methodology that aims to automate the commonly used workflow of copying, pasting, and modifying code available online. Here, the programmer starts by writing a "draft" that mixes unfinished code, natural language comments, and correctness requirements in the form of test cases or API call sequence constraints. A program synthesizer that interacts with a large, searchable database of program snippets is used to automatically complete the draft into a program that meets the requirements. The synthesis process happens in two stages. First, the synthesizer identifies a small number of programs in the database that are relevant to the synthesis task. Next it uses an enumerative search to systematically fill the draft with expressions and statements from these relevant programs. The resulting program is returned to the programmer, who can modify it and possibly invoke additional rounds of synthesis. We present an implementation of program splicing for the Java programming language. The implementation uses a corpus of over 3.5 million procedures from an open-source software repository. Our evaluation uses the system in a suite of everyday programming tasks, and includes a comparison with a state-of-the-art competing approach as well as a user study. The results point to the broad scope and scalability of program splicing and indicate that the approach can significantly boost programmer productivity.

==> sketch.tex <==
\lstset{ %
  aboveskip=20pt,
  belowskip=20pt,
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\fontsize{6}{7}\selectfont\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  % captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=[ANSI]C,                 % the language of the code
  morekeywords={*,??,...},            % if you want to add more keywords to the set
  numbers=none,                    % where to put the line-numbers; possible values are (none, left, right)
  % numbersep=5pt,                   % how far the line-numbers are from the code
  % numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
  % rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  % stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  % stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  % title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.28\textwidth}
      \begin{lstlisting}
int sieve_prime(int num) {
  // use sieve of erathosthenes
  // to test primality
  int prime[105], i, j;
  // build the table
  ??;
  return prime[num];
}
      \end{lstlisting}
      \caption{Primality Testing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
      \begin{lstlisting}
/**
* This is the floyd warshall algorithm.
* All-pairs shortest path
*/
int floyd_warshall(int dist[5][5],
                   int start,
                   int end,
                   int n) {
  int i, j, k;
  // This is the floyd warshall
  // algorithm. All-pairs shortest path
  ??;
  return dist[start][end];
}
      \end{lstlisting}
      \caption{Floyd Warshall}
    \end{subfigure}
    \begin{subfigure}[b]{0.28\textwidth}
      \begin{lstlisting}
void qsort(int a[], int l, int r) {
  // quick sort
  int i, j, x, w;

  // partition
  ??;

  if (l < j) qsort(a, l,j);
  if (i < r) qsort(a, i, r);
}
      \end{lstlisting}
      \caption{Quick Sort}
    \end{subfigure}

    \begin{subfigure}[b]{0.45\textwidth}
      \begin{lstlisting}
void lcs( int *X, int *Y, int m, int n, int *result) {
  // longest common subsequence
  int L[15][15], i, j, index, s;
  // build the table here
  ??;
  index = L[m][n]; s=index; i = m; j = n;
  while (i > 0 && j > 0) {
	if (X[i-1] == Y[j-1]) {
      // Put current character in result
      result[index-1] = X[i-1]; 
      // reduce values of i, j and index
	  i--; j--; index--;     
    } else if (L[i-1][j] > L[i][j-1])
        i--;
      else
		j--;
	}
}
      \end{lstlisting}
      \caption{LCS}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
      \begin{lstlisting}
/**
* This function takes a string and then see if
* after a character is removed, the resulting
* string is a palindrome. 
*/
int palindrome(char s[]) {
  int size = strlen(s);
  char substr[20];
  // find palindrome for a string
  for(int i = 0; i < size; ++i) {
	// remove a char from the string
	int pos = 0;
	for(int j = 0; j < size; ++j) 
	  if(i != j) 
		substr[pos++] = s[j];
      substr[pos] = '\0';
      // test whether the new string is a palindrome
	  int sublen = strlen(substr);
	  int is_palindrome = 1;
      ??;
      if(is_palindrome) return i;
    }
  return -1;
}
      \end{lstlisting}
      \caption{Palindrome}
    \end{subfigure}
    
    \begin{subfigure}[b]{\textwidth}
      \begin{lstlisting}[multicols=2]
int prims(int graph[5][5], int cluster[], int nsize, int csize) {
	int key[5];   // Key values used to pick minimum weight edge in cut
	int used[5] = {0};
	int cluster_size = 0;
	int u;
	int min_dist;
	int i;
	int count;
	
	// Initialize all keys as INFINITE
	for (i = 0; i < nsize; i++)
		key[i] = 100000;
	
	// Always include first 1st vertex in MST.
	key[0] = 0;     // Make key 0 so that this vertex is picked as first vertex
	used[0] = 1;
	cluster[cluster_size++] = 0;
	
	// The MST will have V vertices
	for (count = 0; count < nsize-1; count++) {
		// Pick thd minimum key vertex from the set of vertices
		// not yet included in MST
		u = -1;
        i = 2147483647;
        for((min_dist = 0); (min_dist < nsize); (min_dist ++))
        {
            if((!used[min_dist]) && (i > key[min_dist]))
            {
                u = min_dist;
                i = key[min_dist];
            }
        }

		if(u == -1) {
			break;
		}
		
		// Add the picked vertex to the cluster
		used[u] = 1;
		cluster[cluster_size++] = u;
		if(cluster_size == csize) {
			return cluster_size;
		}

        // update the node distances
		??;
	}
	
	return cluster_size;
}
      \end{lstlisting}
      \caption{Prims}
    \end{subfigure}
    \caption{Sketches used for experiments}
    \label{fig:sketches}
\end{figure*}

